An optimal control strategy to design passive thermal cloaks of arbitrary shape

In this paper we describe a numerical framework for achieving passive thermal cloaking of arbitrary shapes in both static and transient regimes. The design strategy is cast as the solution of an optimal control problem (OCP) for the heat equation where the coefficients of the thermal diffusivity matrix take the role of control functions and the distance between the uncloaked and the cloaked field is minimized in a suitable observation domain. The control actions enter bilinearly in the heat equation, thus making the resulting OCP nonlinear, and its analysis nontrivial. We show that optimal diffusivity coefficients exist both for the static and the transient case; we derive a system of first-order necessary optimality conditions; finally, we carry out their numerical approximation using the Finite Element Method. A series of numerical test cases assess the capability of our strategy to tackle passive thermal cloaking of arbitrarily complex two-dimensional objects.

==> sections/thm.tex <==

In this Section we prove an existence theorem regarding the existence of at least one optimal control for both the static and time-dependent problem. The proof of the main theorems is provided in the main text while the proofs of theorems on well-posedness of the state problems and differentiability of the control-to-state maps are provided in the Appendix \crl{ADD REF}

The analysis of the problem is carried out considering a unique isotropic control $u$ acting through an identity matrix $I$. The extension to the case with three control terms is immediate since we are working in linear vector spaces . Here $\Omega\subset\mathbb{R}^2$ is bounded domain with $\partial{\Omega}$ Lipschitz. The following minimization problem is treated
\begin{equation} \label{functional_analysis}
    \min\limits_{u,q} J(u,q) = \frac{1}{2}\int_{\Omega_{obs}} (q-z)^2 \,d\Omega + \frac{\beta}{2} \int_{\Omega_{c}} u^2 \,d\Omega
\end{equation}
\begin{equation} \label{pde_analysis}
    \textrm{$subject$ $to$} 
    \begin{cases}
    \begin{array}{ll}
    \nabla{}\cdot\{-[(\mu+u\chi_{c}(\textbf{x}))I ]{\nabla{q(\textbf{x})}}\}=s(\textbf{x} )&\text{in $\Omega$}
          \\
          q(\textbf{x}) = T_{0}&\text{on $\Gamma_{o}$}
          \\
          -\mu\nabla{q}\cdot \textbf{n}+\alpha q(\textbf{x}) = 0&\text{on $\partial\Omega_{un}=\Gamma_{d}$}.
    \end{array}
    \end{cases}
\end{equation}

 The weak form of this problem is: 
\begin{equation} \label{weak_fomulation_analysis}
    \text{$find$ $\tilde{q}\in V$: $a(\tilde{q},v)$} = Fv \quad \forall v\in V
\end{equation}

\noindent With:

\begin{equation} \label{bilinear_form_and_linear_functional}
    \text{$a(q,p)$} = \int_{\Omega} (\mu + u\chi_{c})I\nabla{q}\cdot\nabla{p} \,d\Omega - \int_{\Gamma_{d}} qp \,d\Gamma,\quad Fv = \tilde{F}v- \text{$a(Rg,v)$},
\end{equation}
$R:H^{1/2}(\Gamma_{o})\rightarrow H^1(\Omega)$ is the lifting operator and the unknown of the problem, for any fixed $u\in \mathcal{U}$, becomes $\tilde{q} = q - Rg$, $\tilde{q}\in V$.
$g$ being the Dirichlet boundary data.

We define the isotropic diffusivity matrix: $K(\textbf{x}) = ( \mu + u \chi_{c}(\textbf{x}))I$ and recall the definition of $H^1(\Omega)$-norm:
\begin{equation}
    \|f\|_{H^1(\Omega)} = \|f\|_{V} = \sqrt{\int_{\Omega} |f|^2 + |\nabla{f}|^2 \,d\Omega} \qquad \forall f\in H^{1}(\Omega). 
\end{equation}
Analogously, the $H^2(\Omega_{c})$-norm is 
\begin{equation*}
    \|f\|_{H^2(\Omega_{c})}^2 = \|f\|_{\mathcal{U}}^2 = \sum_{|\alpha|\leq 2} \int_{\Omega_{c}} |D^{\alpha}f|^2 \,d\Omega,\quad\forall f\in H^2(\Omega_{c}). 
\end{equation*}
As a preliminary result, we start by proving the well-posedness of the state dynamics for every control $u \in \mathcal{U}$. We can prove the following
\begin{theorem}[Well posedness of the state problem \ref{pde_analysis}] \label{Theorem_1}\ \\
Assume that $u\in\mathcal{U}$, with $\mathcal{U}=H^{2}(\Omega_{c})$, is such that the matrix $K$ is positive definite over $\Omega_{c}$.
Then there exists a unique weak solution $q\in H^{1}(\Omega)$ to problem \eqref{pde_analysis}. Furthermore it holds the a-priori-bound
\begin{equation} \label{lax-milgram bound}
    \|\tilde{q}\|_{V}\leq \frac{|s| + \tilde{M}\|Rg\|_{V}}{\tilde{\alpha}}.
\end{equation}
\begin{proof}
    see the Appendix \ref{proofTHM1}.
\end{proof}

\end{theorem}


We will denote from now on $\tilde{q}=q$. 

In order to prove existence of optimal controls and derive the associated system of first-order necessary conditions for optimality we need to show that the control-to-state map is differentiable in a suitable sense.
We now define the control-to-state map that associates to every $u\in \mathcal{U}$ an element of $V$: $\Theta:\mathcal{U}\rightarrow V$.
We want to prove that the control to state map $q=\Theta(u)$ is Fréchet differentiable. We need to show that for every $u\in \mathcal{U}$ there exists an operator $\Theta'\in\mathcal{L}(\mathcal{U},\mathcal{L}(\mathcal{U},V))$ such that, for all $h\in \mathcal{U}$ such that $u+h\in \mathcal{U}$, the following relation holds:
\begin{equation*}
    \Theta(u+h) - \Theta(u) = \Theta'(u)h + R(u,h),
\end{equation*}
where $R(u,h)=o(\|h\|_{\mathcal{U}})$ for $\|h\|_{\mathcal{U}}\rightarrow 0$. We can prove the following 

\begin{theorem}[Differentiability of the control to state map] \label{Theorem_2}\ \\
    The $control-to-state$ map: $\Theta: \mathcal{U}\rightarrow V$ is Fréchet differentiable and the directional derivative:
    
    \noindent $z = \Theta'(u)h$ at $u\in \mathcal{U}$ in the direction $h\in\mathcal{U}$ is: 

\begin{equation*}
 \begin{cases}
 \begin{array}{ll}
        - \nabla{}\cdot[  (\mu+u\chi_{c})\nabla{z}] = \nabla{}\cdot[h\chi_{c}\nabla{q}(u)] & \text{in $\Omega$} \\
        z = 0 &  \text{on $\Gamma_{o}$}\\
        -\mu\nabla{z}\cdot \textbf{n} + z = 0 & \text{on $\Gamma_{d}$}
    \end{array}
    \end{cases}\,.
\end{equation*}
\begin{proof}
    see the Appendix \ref{proofTHM2}.
\end{proof}

\end{theorem}

We can now show that for the OCP \eqref{functional_analysis}-\eqref{pde_analysis} there exists at least an optimal control.
\begin{theorem}[Existence of an optimal control]\ \\ 
    There exists at least an optimal solution $(\hat{q},\hat{u})\in V \times \mathcal{U}$ of the optimal control problem \eqref{functional_analysis}- \eqref{pde_analysis}.

\begin{proof}
    $Theorem$ \ref{Theorem_1} already warrants that, for all fixed $u\in \mathcal{U}$, there exists a unique state $q=q(u)$. By $theorem$ \ref{Theorem_2} we have proved the $\mathcal{F}$-differentiability of the control-to-state map.
    First of all, we rewrite the state equation as an abstract operator: $G: V \times \mathcal{U} \rightarrow V^\star$, given by
\begin{equation*}
    G(q,u) = Aq + B(u,q) - s,
\end{equation*}
\begin{equation*}
    G(q,u) = Aq + B(u,q) - s\quad .
\end{equation*}
where we have split the bilinear form $a(q,\phi)$ in this way:
\begin{equation*}
    a(q,\phi) = \langle Aq + B(u,q) , \phi \rangle 
\end{equation*}
with $A:V\rightarrow{}V^\star$,
\begin{equation*}
     \langle Aq,\phi\rangle = \mu\int_{\Omega} \nabla{\phi} \cdot \nabla{q} \,d\Omega - \int_{\Gamma_{d}} q\phi \,d\Gamma 
\end{equation*}
and $B:\mathcal{U}\times V\rightarrow{}V^\star$,
\begin{equation*}
     \langle B(u,q),\phi\rangle = \int_{\Omega_{c}} u\nabla{q} \cdot \nabla{\phi} \,d\Omega;
\end{equation*}
finally,
\begin{equation*}
    \langle s,\phi\rangle = \int_{\Omega} s\phi \,d\Omega.
\end{equation*}
The action of the state equation on an element $\phi\in V$ is therefore
\begin{equation*}
        \langle G(q,u),\phi\rangle =\langle Aq + B(u,q) - s , \phi \rangle  = 0.
\end{equation*}
The proof is made by applying Theorem 9.4 of \textit{\cite{manzonioptimal}}, one has to check that:
\begin{enumerate}
    \item $\inf\limits_{(q,u)} J(q,u)= \zeta > -\infty$ and the set of feasible points is nonempty;
    \item a minimizing sequence $\{q_{k},u_{k}\}$ is bounded in $V\times\mathcal{U}$;
    \item the set of feasible points is weakly sequentially closed in $V\times\mathcal{U}$;
    \item $J$ is sequentially weakly lower semicontinuous. 
\end{enumerate}
One can prove that our problems satisfy these four assumptions
    \begin{enumerate}
        \item The cost functional is bounded from below, since
        
        \begin{equation}
        \inf\limits_{(q,u)} J(q,u)= \zeta > -\infty,
    \end{equation}
    and the set of feasible points is non-empty since $J(q,u) \geq 0 $.
       \item A minimizing sequence: $\{(q_{k},u_{k})\}_{k\in \mathbb{N}}\subseteq V\times \mathcal{U}$ such that $J(y_{k},u_{k}) \rightarrow \zeta$ and 
    $G(y_{k},u_{k})=0\quad k\in\mathbb{N}$ is bounded. This follows from the definition of $\mathcal{U}$ and the bound \eqref{lax-milgram bound}. 
    \item To prove that the set of feasible points is $weakly$ sequentially closed in $Y\times \mathcal{U}$ we consider the following sequences:
    \begin{equation*}
    u_{n} \rightharpoonup u \quad \textrm{$in$  $\mathcal{U}$},\quad q_{n} \rightharpoonup q \quad \textrm{$in$ $V$},\quad Aq_{n}  \overset{\star}{\rightharpoonup} \Lambda \quad in\: V^\star,\quad B(u_{n},q_{n})  \overset{\star}{\rightharpoonup} \Phi \quad in\: V^\star. 
    \end{equation*}
    
    We have that $(q,u)\in V\times \mathcal{U}$ since $V$ and $\mathcal{U}$ are $weakly$ sequentially closed.
    We have that $(q,u)\in V\times \mathcal{U}$ since $V$ and $\mathcal{U}$ are $weakly$ sequentially closed.
    Using this definition we, first of all, prove that $\Lambda = Aq$, showing that: 
    \begin{equation*} \label{1weak1}
        \langle Aq_{n} - Aq , \phi \rangle  \rightarrow 0 \quad \forall\phi\in V.
    \end{equation*}
    This amounts to show that
    \begin{equation*}
        \mu\int_{\Omega}( \nabla{q}_{n}-\nabla{q})\cdot\nabla{\phi}\,d\Omega - \int_{\Gamma_{d}} (q_{n}-q)\phi \,d\Gamma \rightarrow 0.
    \end{equation*}
    We consider in this step the equivalent definition of scalar product in $V=H^1_{\Gamma_{o}}(\Omega)$:
    \begin{equation*}
        (u,v)_{V} = \int_{\Omega} \nabla{u}\cdot\nabla{v} \,d\Omega 
    \end{equation*}
    
    and so we can exploit the $weak$ convergence in the reflexive space $V$. In particular, we have: 
    \begin{equation*}
        q_{n} \rightharpoonup q \quad \text{in $V$} \iff  \nabla{q}_{n} \rightharpoonup \nabla{q} \quad \text{in $L^2(\Omega)$}.
    \end{equation*}
    Furthermore by the continuity of the trace operator (see e.g. \textit{\cite{manzonioptimal}, Appendix A}) holds: 
    
    $q_{n}\rightharpoonup q$ in $L^2(\Gamma_{d})$. 
    
    We now prove that for each: $\phi\in V$:
    \begin{equation}
        \langle B(u_{n},q_{n}),\phi\rangle  \rightarrow  \langle B(u,q),\phi\rangle  
    \end{equation}
    that is:
    \begin{equation} \label{convergence_u_n_u}
        \int_{\Omega_{c}} (u_{n}\nabla{q_{n}}-u\nabla{q})\cdot \nabla{\phi} \,d\Omega   \rightarrow 0 \qquad for\:n\rightarrow\infty
    \end{equation}
        
    and so $B(u,q)=\Phi$.     
        
    \eqref{convergence_u_n_u} is equivalent to show:
    \begin{equation} \label{convergence_u_n_u_expanded}
        \int_{\Omega_{c}} \nabla{q}_{n}\cdot\nabla{\phi}(u_{n}-u) \,d\Omega + \int_{\Omega_{c}} ( \nabla{q_{n}} - \nabla{q} ) \cdot \nabla{\phi}u \,d\Omega  \rightarrow 0 \qquad for\:n\rightarrow\infty
    \end{equation} 
        
    For what concerns the first term of \eqref{convergence_u_n_u_expanded}:
    
    \begin{equation*}
        \lim_{n\to \infty} \int_{\Omega_{c}} ( u - u_{n} ) \nabla{q}_{n} \cdot \nabla{\phi} \,d\Omega = 0 
    \end{equation*}
    
    this can be proven using the compact embedding in dimension $n=2,3$:
    
    
    $H^2(\Omega_{c})\hookrightarrow \hookrightarrow  L^{\infty}(\Omega_{c})$ in the following way:
    \begin{equation*}
        \lvert{}\int_{\Omega_{c}} (u-u_{n})\nabla{q}_{n}\cdot{\nabla{\phi}} \,d\Omega \rvert{} \leq \|u-u_{n}\|_{L^{\infty}(\Omega_{c})}\|\nabla{\phi}\|_{L^2(\Omega)}\|\nabla{q}_{n}\|_{L^2(\Omega)} \rightarrow 0
    \end{equation*}
    where $\|u-u_{n}\|_{L^{\infty}(\Omega_{c})}\rightarrow 0$ and $\|\nabla{q}_{n}\|_{L^2(\Omega)}\leq M_{weak}$, with $M_{weak}>0$ since every weak convergent sequence is bounded. 
        
    For the second term in \eqref{convergence_u_n_u_expanded} we have:
    
    \begin{equation} \label{weakconv1}
        \lim_{n\to \infty} |\int_{\Omega_{c}} ( \nabla{q_{n}} - \nabla{q} ) \cdot \nabla{\phi}u \,d\Omega| \rightarrow 0 
    \end{equation}
    
    here we use again the fact that $\nabla{q_{n}} \rightharpoonup \nabla{q}$ in $L^2(\Omega)$ with the information that 
    
    $\nabla{\phi}u = \psi \in L^2(\Omega)$ since $\phi \in H^1_{\Gamma_{d}}(\Omega)$ and $u\in \mathcal{U}\subseteq L^{\infty}(\Omega_{c})$. 
    
    Gathering all this information together we can conclude that $G(q,u)=0$ in $V^\star$ and so by the arbitrariness of the sequence taken we have that the set of feasible points is $weakly$ sequentially closed.
    \item $J(q,u)$ is convex and continuous in $V\times\mathcal{U}$.
    We can so conclude that $J$ is lower semi-continuous with respect to the weak convergence:
    \begin{equation*}
        J(q,u) \leq \liminf\limits_{n\rightarrow \infty} J(q_{n},u_{n}) = \zeta.
    \end{equation*}
    \end{enumerate}
    We can so infer the existence of an optimal solution $(\hat{q},\hat{u})$.
\end{proof}
\end{theorem}

We now turn to the analysis of the time-dependent problem where we assume to be able to change the diffusivity of the material inside the cloak both in space and in time. We start by formulating the time-dependent problem and then prove that analogous results as for the stationary configuration hold. The time-dependent OCP can be written as
\begin{equation} \label{functional_td_analysis}
    \min\limits_{u(t),q(t)} J(u(t),q(t)) = \frac{1}{2}\int_{0}^{T}\int_{\Omega_{obs}} (q(t)-z(t))^2 \,d\Omega dt+ \frac{\beta}{2} \int_{0}^{T}\int_{\Omega_{c}} u(t)^2 \,d\Omega dt
\end{equation}
\begin{equation} \label{pde_td_analysis}
    \textrm{$subject$ $to$} 
    \begin{cases}
    \begin{array}{ll}
    \frac{\partial{q}}{\partial{t}}(\textbf{x},t) + \nabla{}\cdot\{-[(\mu+ \\
    u(\textbf{x},t)\chi_{c}(\textbf{x}))I ]{\nabla{q(\textbf{x},t)}}\}=s(\textbf{x} )&\text{in $\Omega\times(0,T)$}
          \\
          q(\textbf{x},t) = 0&\text{on $\Gamma_{o}\times(0,T)$}
          \\
          -\mu\nabla{q}\cdot \textbf{n}+\alpha q(\textbf{x}) = 0&\text{on $\partial\Omega_{un}=\Gamma_{d}\times(0,T)$} \\
          q(\textbf{x},0) = q_{0} = 0 &\text{in $\Omega\times\{0\}$}.
    \end{array}
    \end{cases}
\end{equation}
We now select suitable functional spaces to deal with the evolution problem involving the state dynamics, we remind the reader to e.g. \cite{evans} Chapter 7 or \cite{manzonioptimal} Chapter 7 for more details on the treatment of linear evolution problems and associated functional spaces. State and control spaces are chosen as  
$Y=H^1(0,T;V,V^{\star})$ and $\mathcal{U} = \{ u \in L^{\infty}(0,T;H^2(\Omega_{c})), \frac{\partial{u}}{\partial{t}}\in L^2(0,T;H^2(\Omega_{c})^{\star})\}$;
$\mathcal{U}$ is a Banach space with the norm
\begin{equation*}
    \|u\|_{\mathcal{U}} = ( \|u\|_{L^{\infty}(0,T;H^2(\Omega_{c}))}^2 + \|\frac{\partial{u}}{\partial{t}}\|_{L^2(0,T;H^2(\Omega_{c})^{\star})}^2 )^{1/2};
\end{equation*}
this can be proven similarly to what was done in \textit{\cite{Chipot_2000}, Theorem 11.4} using the embedding: 
\begin{equation*}
     L^{\infty}(0,T;H^{2}(\Omega_{c}))\hookrightarrow \mathcal{D}'(0,T;H^{2}(\Omega_{c})) \hookrightarrow \mathcal{D}'(0,T;H^{2}(\Omega_{c})^{\star}).
\end{equation*}
We define the parabolic operator: $\mathcal{P}$ as follows:
\begin{equation*}
    \mathcal{P}q = \frac{\partial{q}}{\partial{t}} + \{[(\mu+u\chi_{c}(\textbf{x}))I]\nabla{q}\}.
\end{equation*}
The following Hilbert triplet is considered: $V\subset H\subset V^{\star}$, with $H=L^2(\Omega)$.
The variational formulation of \eqref{pde_td_analysis} is the following: 
\begin{equation} \label{weak_td_problem}
\begin{cases}
\begin{array}{ll}
    \langle\frac{\partial{q}}{\partial{t}}(t),\phi\rangle  + a(q(t),\phi)=\langle s,\phi\rangle  & \text{$\forall \phi\in V$, in $\mathcal{D}'[0,T)$} \\
    q(0) = q_{0}\in H, 
\end{array}
\end{cases}
\end{equation}
meaning that
\begin{align} \label{extended_weak_formulation}
    &-\int_{0}^{T} (q(t),\phi)_{H}\psi'(t)dt - (q(0),\phi)_{H}\psi(0) + \int_{0}^{T} a(q(t),\phi)\psi(t)dt = \\
    &\int_{0}^{T} \langle f(t),\phi \rangle \psi(t)dt \quad \forall \phi\in V, \quad \forall \psi(t)\in \mathcal{D}[0,T),
\end{align}
where the bilinear form $a(\cdot,\cdot)$ has already been defined in \eqref{bilinear_form_and_linear_functional}. 
Given that $s\in L^2(0,T;V^{\star})$, $q_{0}\in H$, the existence and uniqueness of a solution for \eqref{weak_td_problem} is guaranteed under the assumption that the operator $\mathcal{P}$ is uniformly parabolic: there exists $\alpha,M>0$: 
\begin{equation*} 
    \alpha\lvert\textbf{y}\rvert^2 \leq \sum_{i,j=1}^{d}k_{i,j}(\textbf{x},t)y_{i}y_{j},\quad 
    \lvert k_{i,j}(\textbf{x},t) \rvert \leq M, \quad \forall \textbf{y}\in\mathbb{R}^d,\quad \text{a.e. in $Q_{c}_{T} = \Omega_{c}\times (0,T)$},
\end{equation*}
where $k_{i,j}$ is the generic term of the matrix $K = ( \mu + u\chi_{c} )I  $.
Under these assumptions there exists a unique $q\in H^1(0,T;V,V^{\star})\subseteq C^{0}([0,T];H)$ weak solution of the abstract equation \eqref{weak_td_problem}. 
Starting from \eqref{extended_weak_formulation}, several estimates on the norm of $q$ can be derived. 
Here the most relevant ones
\begin{subnumcases}{}
   \|q\|_{L^2(0,T;V)}^2 \leq K_{2}( s , q(0) , \tilde{\alpha}, T ) \label{L2_V}\\
   \|q\|_{Y}^2 \leq  K_{2}(s,q(0),\tilde{\alpha},T) + 2\{ \tilde{M}^2[K_{2}(s,q(0),\tilde{\alpha},T)]+|s|^2 T \}\label{Y_norm},
\end{subnumcases}
where: $K(s,q(0),\tilde{\alpha},T)= \frac{|s|^2T}{\tilde{\alpha}} + \|q(0)\|_{L^2(\Omega)}^2>0$, $K_{2}( s , q(0) , \tilde{\alpha} , T)= \frac{1}{\tilde{\alpha}} \{ |s|K(s,q(0),\tilde{\alpha},T)T + \frac{1}{2} \|q(0)\|_{L^2(\Omega)}^2 \}$, $\tilde{M},\tilde{\alpha}$ being the continuity and coercivity constants of the form  \eqref{bilinear_form_and_linear_functional}. Using similar arguments as in the proof of the differentiability of the contorl-to-state map in the stationary case we can prove differentiability of the control-to-state map for the time-dependent case. We have the following

\begin{theorem}[Differentiability of the control to state map] \label{Theorem_4}\ \\
The $control-to-state$ map: $\Theta: \mathcal{U}\rightarrow Y$ is Fréchet differentiable and the directional derivative: $z = \Theta'(u)h\in Y$ at $u\in \mathcal{U}$ in the direction $h\in\mathcal{U}$ is: 

\begin{equation}\label{pde_z_td_analysis}
 \begin{cases}
 \begin{array}{ll}
        \frac{\partial{z}}{\partial{t}} + \nabla{}\cdot[ - (\mu+u\chi_{c})\nabla{z}] = \nabla{}\cdot[h\chi_{c}\nabla{q}(u)] & in \:\:\Omega \times (0,T) \\
        z = 0 & on \:\: \Gamma_{0}\times(0,T)\\
        -\mu\nabla{z}\cdot \textbf{n} + z = 0 & on \:\: \Gamma_{R}\times(0,T)\\
        z(\textbf{x},0) = 0 & in \:\: \Omega\times \{0\}.
    \end{array}
    \end{cases}
\end{equation}
\begin{proof}
    see the Appendix \ref{proofTHM4}.
\end{proof}
\end{theorem}

In order to prove the existence of an optimal pair $(\hat{q},\hat{u})\in Y\times\mathcal{U}$, the state equation is recast in the dual space $V^\star$ for a.e. $t$ by introducing the operator $G:V\times \mathcal{U} \rightarrow V^\star$ given by
\begin{equation*}
    G(q,u) = \begin{pmatrix} \dot{q}(t) + Aq(t) + B(u(t),q(t)) - s \\
    q(0) = q_{0}
    \end{pmatrix}.
\end{equation*} 
The bilinear form $a(q(t),\phi)$ can be split so that
\begin{equation*}
    a(q(t),\phi) = \langle Aq(t) + B(u(t),q(t)) , \phi \rangle  
\end{equation*}
with $A:L^{2}(0,T;V)\rightarrow{}L^{2}(0,T;V^\star)$:
\begin{equation*}
     \langle (Aq)(t),\phi(t)\rangle  = \mu\int_{\Omega} \nabla{\phi} \cdot \nabla{q}(t)  \,d\Omega - \int_{\Gamma_{R}} q(t)\phi \,d\Omega,
\end{equation*}
while the control operator $B:\mathcal{U}\times L^{2}(0,T;V)\rightarrow{}L^{2}(0,T;V^\star)$ is defined as
\begin{equation*}
     \langle B(u(t),q(t)),\phi(t)\rangle  = \int_{\Omega_{c}} u(t)\nabla{q}(t) \cdot \nabla{\phi}(t) \,d\Omega
\end{equation*}
We can now prove an existence theorem showing that there exist at least an optimal solution to the time-dependent problem. We have the following
\begin{theorem}[Existence of an optimal control]\ \\ 
    There exists at least an optimal solution $(\hat{q},\hat{u})\in V \times \mathcal{Y}$ of the optimal control problem \eqref{functional_td_analysis}- \eqref{pde_td_analysis}.
\begin{proof} (Sketch)
    We use Theorem 9.4 of \textit{\cite{manzonioptimal}}.
    The hypothesis $(i)$, $(ii)$, $(iv)$ are trivially satisfied. Notice that \eqref{Y_norm} bounds the $\|\cdot\|_{H^1(0,T;V,V^\star)}$-norm.
    
    Hypothesis $(ii)$ asks to show that the set of feasible points is $weakly^\star$ sequentially closed in $Y\times \mathcal{U}$. The following sequences are considered:
    \begin{align*}
    \begin{split}
    &u_{n} \overset{\star}{\rightharpoonup} u \quad \textrm{$in$  $\mathcal{U}$}, \quad q_{n} \rightharpoonup q \quad \textrm{$in$ $Y$}, \quad Aq_{n} \overset{\star}{\rightharpoonup} \Xi \quad in\: L^2(0,T;V^\star), \quad B(u_{n},q_{n})  \overset{\star}{\rightharpoonup} \Phi \quad in\: L^2(0,T;V^\star)
    \end{split}
    \end{align*}
    with $G(q_{n},u_{n}) = 0\quad \forall n\in\mathbb{N}$.
    $(q,u)\in Y\times \mathcal{U}$ since $\mathcal{U}$ is $weakly^\star$ sequentially closed. The proof that $G(q,u)=0$ in $W$ is done in three substeps:
     \begin{itemize}
        \item $Aq=\Xi$ since $\nabla{q_{n}}\rightharpoonup\nabla{q}$ $in$ $L^2(0,T;L^2(\Omega))$ and $q_{n}\rightharpoonup q$ $in$ $L^2(0,T;L^2(\Gamma_{R}))$.
        \item $B(u,q)=\Phi$, since, $\forall \phi\in L^2(0,T;V)$
        \begin{equation*}
            \int_{0}^{T} \langle B(u_{n}(t),q_{n}(t)),\phi(t)\rangle  dt \rightarrow \int_{0}^{T} \langle B(u(t),q(t)),\phi(t)\rangle  dt,
        \end{equation*}
        that is,
        \begin{equation} \label{B_equal_phi}
            \int_{0}^{T} \int_{\Omega_{c}} (u_{n}(t)\nabla{q_{n}(t)}-u(t)\nabla{q}(t))\cdot \nabla{\phi}(t) \,d\Omega dt  \rightarrow 0,
        \end{equation}
        adding and subtracting to \eqref{B_equal_phi} $u\nabla{q}_{n}\cdot\nabla{\phi}$ it suffices to note that     
        \begin{equation*}
            \lim_{n\to \infty} \int_{0}^{T}\int_{\Omega_{c}} ( u(t) - u_{n}(t) ) \nabla{q}(t) \cdot \nabla{\phi}(t) \,d\Omega dt = 0 
        \end{equation*}
        
        that can be proven exploiting the compact embedding $H^{2}(\Omega_{c})\hookrightarrow\hookrightarrow L^{\infty}(\Omega_{c})$ in dimension $n=2,3$.
         In fact, using Aubin-Lions Lemma (see e.g. \cite{AubinLions,Chen_2013}) holds the following embedding
        $\mathcal{U}\hookrightarrow \hookrightarrow L^{\infty}(0,T;L^{\infty}(\Omega_{c}))$. We then have:
        \begin{align*}
        \begin{split}
            &\lvert{}\int_{0}^{T}\int_{\Omega_{c}} (u(t)-u_{n}(t))\nabla{q}_{n}(t)\cdot{\nabla{\phi}}(t) \,d\Omega dt \rvert{} \leq \\
            &\leq \|u-u_{n}\|_{L^{\infty}(0,T;L^{\infty}(\Omega_{c}))}\|\nabla{\phi}\|_{L^2(0,T;L^2(\Omega))}\|\nabla{q}_{n}\|_{L^2(0,T;L^2(\Omega))} \rightarrow 0
        \end{split}
        \end{align*}
        where $\|u-u_{n}\|_{L^{\infty}(0,T;L^{\infty}(\Omega_{c}))}\rightarrow 0$. 
        
        Similarly 
        \begin{equation*} 
            \int_{0}^{T}\int_{\Omega_{c}} ( \nabla{q_{n}}(t) - \nabla{q}(t) ) \cdot \nabla{\phi}(t)u(t) \,d\Omega dt 
        \end{equation*}
        vanishes using the fact that 
        $u\in \mathcal{U}\subseteq L^{\infty}(0,T;L^{\infty}(\Omega_{c}))$ and then $\nabla{\phi}u\in L^2(0,T;L^2(\Omega))$, and since $\nabla{q}_{n}\rightharpoonup \nabla{q}$ in $L^2(0,T;L^2(\Omega)$.
        \item 
        \begin{equation} \label{q_n_to_q_dot}
            \int_{0}^{T} \langle\dot{q}_{n}(t),\phi\rangle dt \rightarrow \int_{0}^{T} \langle\dot{q}(t),\phi\rangle dt \qquad \phi\in L^2(0,T;V)
        \end{equation}
        integrating by parts with: $\phi = w\psi$, $w\in V,\psi\in \mathcal{D}[0,T)$ we derive
        \begin{equation*}
            \int_{0}^{T} \langle\dot{q}_{n}(t),\phi\rangle dt = -\int_{0}^{T} (q_{n},w)_{L^2(\Omega)}\psi'(t) dt - (q_{n}(0),w)_{L^2(\Omega)}\psi(0),
        \end{equation*}
        analogously,
        \begin{equation*}
            \int_{0}^{T} \langle\dot{q}(t),\phi\rangle dt = -\int_{0}^{T} (q,w)_{L^2(\Omega)}\psi'(t) dt - (q(0),w)_{L^2(\Omega)}\psi(0);
        \end{equation*}
        \eqref{q_n_to_q_dot} is proved once we notice that since $q_{n} \rightharpoonup q$ in $Y$, we have that $q_{n}(0) \rightharpoonup q(0)$ in $L^2(\Omega)$, furthermore $w\psi'\in L^2(0,T;V)$ and $w\psi(0)\in V$. 
        \end{itemize}
        
    Gathering all this information together we can conclude that $G(q,u)=0$ in $W$ \crl{$V^{\star}$ ?} and so, by the arbitrariness of the sequence taken, we have that the set of feasible points is $weakly^\star$ sequentially closed.
\end{proof}
\end{theorem}

Due to the nature of $\mathcal{U}$, $Y\times \mathcal{U}$ is not a reflexive space, however, being the dual of the separable space $H^1(0,T;V^\star,V)\times \Upsilon$, the theorem can still be applied, where the space $\Upsilon$ is defined as
\begin{equation*}
    \Upsilon= \{f\in L^{1}(0,T;H^2(\Omega_{c})^{\star}): \frac{\partial{f}}{\partial{t}}\in L^2(0,T;H^2(\Omega_{c})^{\star\star})\}.
\end{equation*}

